Massive Multi-Document Summarization of Product Reviews with Weak Supervision

Product reviews summarization is a type of Multi-Document Summarization (MDS) task in which the summarized document sets are often far larger than in traditional MDS (up to tens of thousands of reviews). We highlight this difference and coin the term "Massive Multi-Document Summarization" (MMDS) to denote an MDS task that involves hundreds of documents or more. Prior work on product reviews summarization considered small samples of the reviews, mainly due to the difficulty of handling massive document sets. We show that summarizing small samples can result in loss of important information and provide misleading evaluation results. We propose a schema for summarizing a massive set of reviews on top of a standard summarization algorithm. Since writing large volumes of reference summaries needed for advanced neural network models is impractical, our solution relies on weak supervision. Finally, we propose an evaluation scheme that is based on multiple crowdsourced reference summaries and aims to capture the massive review collection. We show that an initial implementation of our schema significantly improves over several baselines in ROUGE scores, and exhibits strong coherence in a manual linguistic quality assessment.

==> figures/figureACRDStats.tex <==
\begin{table}[h]
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{l|c}
			\textbf{Size of Review Set} & \textbf{Number of Products} \\ 
			1-9 &  \\
			10-99 & \\
		\end{tabular}%
	}
	\caption{Statistics on the full data we use as part of our analyses, training, testing and evaluation. This data is sampled from the Amazon Customer Reviews Dataset.}
	\label{tab_acrd_stats}
\end{table}

==> figures/figureSummaryExampleFull.tex <==
\begin{figure}[]
    \small    
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|p{\columnwidth}|} \hline \\
        %Electronics - B006SUWZH2 \\ 
        \normalsize
        \textbf{Product: ``Memorex Portable CD Boombox with AM FM Radio'' (Electronics)} \\ \\
        \textbf{Reference Summary 1 (crowdsourced)} \\
        Bombox for analog CD playback has AM and FM radio ideal for a picnic and easy to handle for children, you can listen to your soft Christmas music in these amazing Bombox that provide optimal sound. \\ \\
        \textbf{Reference Summary 2 (crowdsourced)} \\
        Excellent customer service. Good sound, light, adorable in appearance almost like an insect. Play CDs beautifully without skipping and has a port to connect your MP3. Great for the price. \\ \\
        \textbf{Reference Summary 3 (crowdsourced)} \\
        It has a good volume, its little in size and very siple to use and carrying anywhere, the sound quality is not the best but it is ok though, i will never regret this buy! \\ \\
        \textbf{Reference Summary 4 (crowdsourced)} \\
        A product that is obtained at an excellent price, has the function of playing CDs and radio transmitting a very acceptable sound. It is a product that is extremely easy to use and enjoy wherever you take it. The negative point is that sometimes the CD is locked. \\ \\
        \textbf{Reference Summary 5 (crowdsourced)} \\
        The reproductive equipment is not very reliable, it has a short duration, and a user always tries to buy the best, the Memorex Portable CD Boombox with AM FM radio has a bad sound, is heard intermittently, it is better to put more money and buy some quality \\ \\
        \textbf{Best F1 Baseline} \\
        This is the perfect size for what I need, sound is good, and it plays the CD'S so clear and well. \\ \\
        \textbf{Multi-Lead-1 Baseline} \\
        I am amazed at the quality of sound coming from this small cd player. Don't waste your money on this one even if it is a low price! horrible! Works very well. I get it...you get what you pay for. Did not have push buttons for radio stations. It's just OK. Radio reception isn't very good but it is tolerable. I purchased this for my girls (3 \& 5 yrs). Works fine. \\ \\
        \textbf{System Summary (\emph{level1-F1} variant)} \\
        It was a gift for my husband. I love this boombox. Very easy to use. This is a great product. It is a great product at a great price. The sound quality is great for the price. Sound is great and sounds like a bose. I am glad i bought it. \\ \\ \hline
    \end{tabular}%
    }
    \caption{Example of automatic summaries and reference summaries for an electronics product.}
    \label{fig_summarySampleFull}
\end{figure}



==> figures/figureSummaryExampleFullWrong.tex <==
\begin{figure}[!ht]
    \small    
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|p{\columnwidth}|} \hline \\
        %Books - 014312417X \\ 
        \normalsize
        \textbf{Product: ``Mastery'' (Books)} \\ \\
        \textbf{Reference Summary 1 (crowdsourced)} \\
        This book describes how to improve your abilities and master a certain craft. It's perfect for those who need to start pursuing their goals, but it could do more to help you figure out those goals. It's good for anyone in their life who wants to understand the journey of mastery and has well written stories. \\ \\
        \textbf{Reference Summary 2 (crowdsourced)} \\
        although it is a book that generally everyone might like, there are certainly flaws in the story because much of the context itself is lost, however it is a story that can be enjoyed \\ \\
        \textbf{Reference Summary 3 (crowdsourced)} \\
        Mastery, written by Robert Greene, reveals that anyone can be an expert in what they set out if they follow in the footsteps of the teachers who have marked the history of mankind. The book has reached the top of the New York Times bestseller list and provides various strategies to continue those ancestral steps. \\ \\
        \textbf{Reference Summary 4 (crowdsourced)} \\
        technically it is a manual of how to define oneself, it is a very interesting book which envelops you that hides some secrets. You can say that the book is self-help \\ \\
        \textbf{Reference Summary 5 (crowdsourced)} \\
        This book turns out to be quite exciting and interesting, from the beginning the listeners feel empathetic and related, although in some moments it turned out to have somewhat repetitive scenes ends up being very pleasing to the listener, The audiobook was narrated excellently by Fred Sanders with a delivery passionate and instructive, this highlights parts of the lives of important characters in universal history, such as Leonardoda Vinci, Marcel Proust, Temple Grandin, among others. \\ \\
        \textbf{Best F1 Baseline} \\
        Mastery was a great read!!! I feel galvanized and inspired!!!! Very useful and I have added to my "tool box" of knowledge! This book is similar to his other book, "48  Laws of Power"  from the perspective  of being able to apply to your personal and professional life. I recommend this book for all ages!! \\ \\
        \textbf{Multi-Lead-1 Baseline} \\
        I started off liking what I was reading until it started to repeat itself,over and over again. Decent book. Another great Robert Green book. One of the ESSENTIAL TEXTS for anyone dedicated to a life of self improvement and bettering your skills. As with all of Robert Greene's books, you have to read it with an open mind. If Malcolm Gladwell had actually spent 10,000 hours studying Outliers, he would have written this much, much better book. Ordered this for a friend of mine. \\ \\
        %sys6 \\
        \textbf{System Summary (\emph{level1-F1} variant)} \\
        I got this book for my husband and he loves it. I have been a fan of the author's blog and this is a great book. I am so glad i did. This is the most important book i have ever read. The book is very well written and has a lot of good information. I would highly recommend this book to anyone. \\ \\ \hline
    \end{tabular}%
    }
    \caption{Example of automatic summaries and reference summaries for the "Mastery" book.}
    \label{fig_summarySampleFull}
\end{figure}



==> figures/figureSummaryExamplesFunny.tex <==
\begin{figure}[]
    \small    
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|p{\columnwidth}|} \hline \\
        %\normalsize
        % DVDs - B00DHHWXYY_17
        \textbf{Product: ``The Great Gatsby'' (DVDs)} \\
        I have read the book several times and have never read the books. This movie is a must see for the family and family. I read the book years ago and loved it. This is one of the best movies ever made . \\ \\
        % DVDs - B0042AGNB4_69
        \textbf{Product: ``Jillian Michaels: 6 Week Six-Pack'' (DVDs)} \\
        I bought this dvd for my husband and she loved it. This is a great workout for the whole family . \\ \\
        % DVDs - B00BWDFP5E_1.dec 
        \textbf{Product: ``Banshee: Season 1'' (DVDs)} \\
        I was hooked on this show. I am still waiting for the next season to come out on dvd. This is one of the best shows on tv. What a disappointment after all the hype. \\ \hline
    \end{tabular}%
    }
    \caption{Problematic summaries generated by our model. They all demonstrate the problem of self-contradiction.}
    \label{fig_summarySamplesFunny}
\end{figure}

==> figures/figureSummaryExamplesWrong.tex <==
\begin{figure}[!ht]
    \small    
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|p{\columnwidth}|} \hline \\
        %DVDs - B0002COTDA \\ 
        \normalsize
        \textbf{Product: ``Columbo - The Complete First Season'' (DVDs)} \\ \\
        \textbf{Reference Summary (crowdsourced)} \\
        This is the uncut version of the first Columbo season. A set that includes five discs that can bring us back to the beginning of this nostalgic series. The only issue is it does not contain any extras, but only the episodes. Oddly, it includes images from the 1990's remake for its main menu. If you are looking for a no frills series of a classic, this one certainly fills that qualification! \\ \\
        \textbf{Best F1 Baseline} \\
        I LOVED COLUMBO SO I GOT THIS 1ST SEASON AND FOUND MYSELF WATCHING IT TO GET FROM ONE EPISODE TO THE NEXT. THE PILOT EPSISODE WAS GREAT AND THIS CHARACTER WAS BORN. I LIKED ALL THE ESPISODES IN THE 1ST SEASON and was only slightly disappointed in one of the episodes. Columbo season one is GREAT TV.....IF YOU liked COLUMBO there will be no disappointment in this purchase. \\ \\
        \textbf{Multi-Lead-1 Baseline} \\
        If you're a diehard Columbo fan you will love the Dvds. It was a happy day when the Columbo series became available on disc. The design of this show is very, very interesting. Great  This is such a cool show...the first half hour you spend watching a carefully planned murder (always by a super rich mogul, what...no poor people kill anyone in the 70's?) Fantastic set! \\ \\
        %sys6 \\
        \textbf{System Summary (\textit{level1-F1} variant)} \\
        The first season of the Columbo series was great. Peter Falk and Lee Grant are great in this movie. I would recommend it to anyone. \\
        \\ \hline
        
        
    \end{tabular}%
    }
    \caption{An actual example of summaries.}
    \label{fig_summarySamples}
\end{figure}



%%\begin{figure}[htb]
%\begin{figure}[]
%    \small    
%    \resizebox{\columnwidth}{!}{%
%    \begin{tabular}{|p{\columnwidth}|} \hline \\
%        %Books - 014312417X \\ 
%        \normalsize
%        \textbf{Product: ``Mastery'' (Books)} \\ \\
%        \textbf{Reference 1} \\
%        This book describes how to improve your abilities and master a certain craft. It's perfect for those who need to start pursuing their goals, but it could do more to help you figure out those goals. It's good for anyone in their life who wants to understand the journey of mastery and has well written stories. \\ \\
%        \textbf{Reference 2} \\
%        although it is a book that generally everyone might like, there are certainly flaws in the story because much of the context itself is lost, however it is a story that can be enjoyed \\ \\
%        \textbf{Reference 3} \\
%        Mastery, written by Robert Greene, reveals that anyone can be an expert in what they set out if they follow in the footsteps of the teachers who have marked the history of mankind. The book has reached the top of the New York Times bestseller list and provides various strategies to continue those ancestral steps. \\ \\
%        \textbf{Reference 4} \\
%        technically it is a manual of how to define oneself, it is a very interesting book which envelops you that hides some secrets. You can say that the book is self-help \\ \\
%        \textbf{Reference 5} \\
%        This book turns out to be quite exciting and interesting, from the beginning the listeners feel empathetic and related, although in some moments it turned out to have somewhat repetitive scenes ends up being very pleasing to the listener, The audiobook was narrated excellently by Fred Sanders with a delivery passionate and instructive, this highlights parts of the lives of important characters in universal history, such as Leonardoda Vinci, Marcel Proust, Temple Grandin, among others. \\ \\
%        \textbf{Best Recall Baseline} \\
%        I like Robert Greene's writing a lot, but can't figure out why he feels compelled to repeat himself so much. Maybe he just likes having these big hefty books to his name, but he could easily cut out about a third of the book with no loss in content. He states most of his points almost verbatim at least two or three times. He did the same thing with Seduction. One thing is for sure - he hammers home his points. \\ \\
%        \textbf{Multi-Lead-1 Baseline} \\
%        I like Robert Greene's writing a lot, but can't figure out why he feels compelled to repeat himself so much. Good book. Great vendor, great book! Very helpful in understanding how to keep learning I'm not sure about the now linear lecture of the book. Purchased as a gift. One of the ESSENTIAL TEXTS for anyone dedicated to a life of self improvement and bettering your skills. \\ \\
%        %sys6 \\
%        \textbf{System Summary} \\
%        I got this book for my husband and he loves it. I have been a fan of the author's blog and this is a great book. I am so glad i did. This is the most important book i have ever read. The book is very well written and has a lot of good information. I would highly recommend this book to anyone. \\
%        \\ \hline
%        
%        
%    \end{tabular}%
%    }
%    \caption{An example of reference summaries, baseline summaries and the summary output by our system. The system variant here is \textit{F1-level1}.}
%    \label{fig_summarySamples}
%\end{figure}

==> figures/tableDataStats.tex <==
\begin{table*}[t]
\centering

\begin{tabular}{l|cccc|cccc}
\multicolumn{1}{c|}{\textbf{}} & \multicolumn{4}{c|}{\textbf{\# Reviews per product}}                  & \multicolumn{4}{c}{\textbf{\# Words in Review}}         \\
\textbf{Category}              & \textbf{Min} & \textbf{Max} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Avg} & \textbf{Med} \\ \hline
Camera                         & 100          & 4652         & 290          & 187          & 1            & 5877         & 67           & 33           \\
Books                          & 100          & 8237         & 324          & 187          & 1            & 8658         & 63           & 27           \\
Electronics                    & 100          & 15334        & 514          & 262          & 1            & 8266         & 55           & 30           \\
Music                          & 100          & 2669         & 249          & 177          & 1            & 8693         & 86           & 37           \\
Toys                           & 100          & 24258        & 318          & 202          & 1            & 4100         & 43           & 26           \\
Video                          & 100          & 4959         & 313          & 210          & 1            & 8401         & 72           & 28           \\ \hline
All                            & 100          & 24258        & 335          & 200          & 1            & 8693         & 63           & 30          
\end{tabular}

\caption{Statistics on the data we base our analysis on from the Amazon Customer Reviews Dataset. 2000 products were randomly chosen in each category.}
\label{tab_dataStats}
\end{table*}

==> figures/tableDatasetStats.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc}
\multicolumn{1}{c|}{\textbf{}} & \textit{(full)} & \textit{(test)} & \multicolumn{8}{c|}{\textbf{\# Reviews}}                                                                                                      & \multicolumn{8}{c}{\textbf{\# Words in Reviews}}                                                                                             \\
\textbf{Category}              & \multicolumn{2}{c|}{\# Products}  & \multicolumn{2}{c|}{\textbf{Min}} & \multicolumn{2}{c|}{\textbf{Max}} & \multicolumn{2}{c|}{\textbf{Avg}} & \multicolumn{2}{c|}{\textbf{Med}} & \multicolumn{2}{c|}{\textbf{Min}} & \multicolumn{2}{c|}{\textbf{Max}} & \multicolumn{2}{c|}{\textbf{Avg}} & \multicolumn{2}{c}{\textbf{Med}} \\ \hline
Camera                         & 2000            & 20              & 100             & 102             & 4652             & 303            & 290             & 174             & 187             & 158             & 1               & 1               & 5877            & 2108            & 67              & 78              & 33              & 45              \\
Books                          & 2000            & 20              & 100             & 102             & 8237             & 425            & 324             & 194             & 187             & 172             & 1               & 1               & 8658            & 2042            & 63              & 65              & 27              & 29              \\
Electronic                     & 2000            & 22              & 100             & 100             & 15334            & 717            & 514             & 235             & 262             & 169             & 1               & 1               & 8266            & 1590            & 55              & 68              & 30              & 37              \\
Music                          & 2000            & 20              & 100             & 100             & 2669             & 445            & 249             & 203             & 177             & 196             & 1               & 1               & 8693            & 2419            & 86              & 94              & 37              & 48              \\
Toys                           & 2000            & 20              & 100             & 100             & 24258            & 489            & 318             & 220             & 202             & 176             & 1               & 1               & 4100            & 1105            & 43              & 53              & 26              & 30              \\
Video                          & 2000            & 21              & 100             & 112             & 4959             & 312            & 313             & 203             & 210             & 193             & 1               & 1               & 8401            & 1964            & 72              & 82              & 28              & 33              \\ \hline
All                            & 12000           & 123             & 100             & 100             & 24258            & 717            & 335             & 205             & 200             & 175             & 1               & 1               & 8693            & 2419            & 63              & 73              & 30              & 36             
\end{tabular}%
}

\caption{Statistics on the data we utilize from the Amazon Customer Reviews Dataset. The left sub-column of each column is on the full data we use, and the right sub-columns are on our test dataset. The training data consists of 1800 products from each category (distinct from the test set).}
\label{tab_datasetStats}
\end{table*}

==> figures/tableDatasetStatsFull.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc}
\multicolumn{1}{c|}{\textbf{}} & \textit{(full)} & \textit{(test)} & \multicolumn{8}{c|}{\textbf{\# Reviews}}                                                                                                      & \multicolumn{8}{c}{\textbf{\# Words in Reviews}}                                                                                             \\
\textbf{Category}              & \multicolumn{2}{c|}{\# Products}  & \multicolumn{2}{c|}{\textbf{Min}} & \multicolumn{2}{c|}{\textbf{Max}} & \multicolumn{2}{c|}{\textbf{Avg}} & \multicolumn{2}{c|}{\textbf{Med}} & \multicolumn{2}{c|}{\textbf{Min}} & \multicolumn{2}{c|}{\textbf{Max}} & \multicolumn{2}{c|}{\textbf{Avg}} & \multicolumn{2}{c}{\textbf{Med}} \\ \hline
Camera                         & 2000            & 20              & 100             & 102             & 4652             & 303            & 290             & 174             & 187             & 158             & 1               & 1               & 5877            & 2108            & 67              & 78              & 33              & 45              \\
Books                          & 2000            & 20              & 100             & 102             & 8237             & 425            & 324             & 194             & 187             & 172             & 1               & 1               & 8658            & 2042            & 63              & 65              & 27              & 29              \\
Electronic                     & 2000            & 22              & 100             & 100             & 15334            & 717            & 514             & 235             & 262             & 169             & 1               & 1               & 8266            & 1590            & 55              & 68              & 30              & 37              \\
Music                          & 2000            & 20              & 100             & 100             & 2669             & 445            & 249             & 203             & 177             & 196             & 1               & 1               & 8693            & 2419            & 86              & 94              & 37              & 48              \\
Toys                           & 2000            & 20              & 100             & 100             & 24258            & 489            & 318             & 220             & 202             & 176             & 1               & 1               & 4100            & 1105            & 43              & 53              & 26              & 30              \\
Video                          & 2000            & 21              & 100             & 112             & 4959             & 312            & 313             & 203             & 210             & 193             & 1               & 1               & 8401            & 1964            & 72              & 82              & 28              & 33              \\ \hline
All                            & 12000           & 123             & 100             & 100             & 24258            & 717            & 335             & 205             & 200             & 175             & 1               & 1               & 8693            & 2419            & 63              & 73              & 30              & 36             
\end{tabular}%
}

\caption{Statistics on the data we utilize from the Amazon Customer Reviews Dataset. The left sub-column of each column is on the full data we use, and the right sub-columns are on our test dataset. The training data consists of 1800 products from each category (distinct from the test set).}
\label{tab_datasetStats}
\end{table*}

==> figures/tablePrevDatasetsFull.tex <==
\begin{table*}[t]
\centering

\begin{tabular}{ll|c|c|c|c}
                           & \textbf{Dataset}     & \textbf{\# sets}       & \thead{\# docs \\ per set}    & \thead{\# tokens \\ per doc} & \thead{\# tokens \\ per ref}                  \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\small Reviews}}   & Opinosis \citep{ganesan2010opinosis}   & 51            & $\dagger$  &  -             &  -                              \\
                           & MeanSum \cite{chu2019meansum}    & 200           & 8              & 70      & -                               \\
                           & Oposum \citep{angelidis2018oposum}     & 60            & 10             & 70      &  -                              \\
                           & MMDS (Ours) & 123           & 205            & 73            & 59 \\ \hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\small News}}      & DUC\textsuperscript{$\ddagger$} 01'-07' (\url{https://duc.nist.gov})  & 45            & 17  & 600     & 200                      \\
                           & TAC\textsuperscript{$\ddagger$} 08'-11' (\url{https://tac.nist.gov}) & 45 & 10             & 600     & 100                            \\
                           & MultiNews \citep{fabbri2019multinews}   & 55K     & 3 & 700     & 260                      \\ \hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{\small Wiki}} & hMDS \cite{zopf2018hMDS}       & 91            & 14       & 2000    & 250                      \\
                           & \citep{Liu2018wikipediaLargeScale}    & 2.3M    & 40       &    -           &  -
\end{tabular}

\caption{Approximate average MDS dataset statistics. \\ $\dagger$ Opinosis concatenates 100 sentences from different reviews. \\ $\ddagger$ In DUC and TAC datasets, values are averaged over all years.}
\label{tab_prev_datasets_stats}
\end{table*}

==> figures/tablePrevDatasetsSimple.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll|c|c|c|c}
                           & \textbf{Dataset}     & \textbf{\# sets}       & \thead{\# docs \\ per set}    & \thead{\# tokens \\ per doc} & \thead{\# tokens \\ per ref}                  \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\small Reviews}}   & Opinosis    & 51            & 100 sents  &  -             &  -                              \\
                           & MeanSum     & 200           & 8              & 70      & -                               \\
                           & Oposum      & 60            & 10             & 70      &  -                              \\
                           & MMDS (Ours) & 123           & 205            & 73            & 59 \\ \hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\small News}}      & DUC 01'-07' & 45            & 17  & 600     & 200                      \\
                           & TAC 08'-11' & 45 & 10             & 600     & 100                            \\
                           & MultiNews   & 55K     & 3 & 700     & 260                      \\ \hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{\small Wiki}} & hMDS        & 91            & 14       & 2000    & 250                      \\
                           & \citep{Liu2018wikipediaLargeScale}    & 2.3M    & 40       &    -           &  -
\end{tabular}%
}
\caption{Approximate average MDS dataset statistics. In DUC and TAC datasets, values are averaged over all years.}
\label{tab_datasetsStats}
\end{table}

==> figures/tableScoresRouge2.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|ll|ll|ll|llllll}
 &  & \multicolumn{6}{c|}{\textbf{Camera}} & \multicolumn{6}{c}{\textbf{Books}} \\ \cline{3-14} 
 & \textbf{Model} & \multicolumn{2}{c|}{\textbf{ROUGE-1}} & \multicolumn{2}{c|}{\textbf{ROUGE-2}} & \multicolumn{2}{c|}{\textbf{ROUGE-L}} & \multicolumn{2}{c|}{\textbf{ROUGE-1}} & \multicolumn{2}{c|}{\textbf{ROUGE-2}} & \multicolumn{2}{c}{\textbf{ROUGE-L}} \\ \hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{\small Model Variants}} & level1-F1 & \textbf{29.25} & (\textpm 1.45) & 5.26 & (\textpm 0.69) & \textbf{17.74} & (\textpm 0.76) & 25.8 & \multicolumn{1}{l|}{(\textpm 1.16)} & \textbf{4.97} & \multicolumn{1}{l|}{(\textpm 0.58)} & 16.48 & (\textpm 0.75) \\
 & level1-Recall & 27.94 & (\textpm 1.53) & \textbf{5.36} & (\textpm 0.61) & 17.18 & (\textpm 0.74) & \textbf{26.9} & \multicolumn{1}{l|}{(\textpm 0.82)} & 4.45 & \multicolumn{1}{l|}{(\textpm 0.43)} & \textbf{17.12} & (\textpm 0.44) \\
 & level1-F2 & 25.94 & (\textpm 2.4) & 4.52 & (\textpm 0.72) & 16.61 & (\textpm 1.15) & 19.76 & \multicolumn{1}{l|}{(\textpm 1.73)} & 3.73 & \multicolumn{1}{l|}{(\textpm 0.52)} & 14.71 & (\textpm 1.0) \\
 & top-F1 & 27.5 & (\textpm 1.88) & 5.06 & (\textpm 0.76) & 17.37 & (\textpm 0.94) & 22.98 & \multicolumn{1}{l|}{(\textpm 1.79)} & 3.85 & \multicolumn{1}{l|}{(\textpm 0.53)} & 15.16 & (\textpm 0.98) \\
 & top-Recall & 18.77 & (\textpm 1.95) & 4.13 & (\textpm 0.5) & 12.62 & (\textpm 0.91) & 22.13 & \multicolumn{1}{l|}{(\textpm 1.28)} & 3.74 & \multicolumn{1}{l|}{(\textpm 0.52)} & 13.77 & (\textpm 0.72) \\
 & top-F2 & 24.72 & (\textpm 2.25) & 4.24 & (\textpm 0.8) & 16.06 & (\textpm 1.05) & 19.12 & \multicolumn{1}{l|}{(\textpm 1.33)} & 3.06 & \multicolumn{1}{l|}{(\textpm 0.52)} & 13.33 & (\textpm 0.94) \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\small Baselines}} & Multi-Lead-1 & 25.37 & (\textpm 1.39) & 3.22 & (\textpm 0.55) & 14.06 & (\textpm 0.75) & 25.03 & \multicolumn{1}{l|}{(\textpm 1.16)} & 3.15 & \multicolumn{1}{l|}{(\textpm 0.45)} & 14.42 & (\textpm 0.67) \\
 & Best Recall & 21.74 & (\textpm 3.15) & 3.1 & (\textpm 0.84) & 12.98 & (\textpm 1.68) & 23.37 & \multicolumn{1}{l|}{(\textpm 1.78)} & 2.7 & \multicolumn{1}{l|}{(\textpm 0.38)} & 13.33 & (\textpm 0.91) \\
 & Cluster + Best Recall & 20.9 & (\textpm 2.76) & 2.48 & (\textpm 0.77) & 13.13 & (\textpm 1.43) & 20.03 & \multicolumn{1}{l|}{(\textpm 2.85)} & 2.54 & \multicolumn{1}{l|}{(\textpm 0.41)} & 13.02 & (\textpm 1.48) \\
 & Best F1 & 18.88 & (\textpm 3.82) & 2.78 & (\textpm 1.01) & 12.4 & (\textpm 2.08) & 19.1 & \multicolumn{1}{l|}{(\textpm 2.82)} & 2.34 & \multicolumn{1}{l|}{(\textpm 0.5)} & 12.37 & (\textpm 1.56) \\
 & Cluster + Best F1 & 17.25 & (\textpm 3.52) & 2.11 & (\textpm 0.69) & 11.24 & (\textpm 2.02) & 18.08 & \multicolumn{1}{l|}{(\textpm 2.86)} & 2.18 & \multicolumn{1}{l|}{(\textpm 0.33)} & 11.96 & (\textpm 1.42)
\end{tabular}%
}
\caption{ROUGE $F_1$ scores on variants of our model and the baselines, on the Camera and Books categories. The model variant name indicates the hierarchical level from which the output summary is taken (level-1 vs. top) and the the metric used for extracting the weak reference of each cluster for training. ROUGE score intervals express 95\% confidence or greater.}
\label{tab_resultsRouge}
\end{table*}




%\begin{table}[]
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{ll|lll}
% & \textbf{Model} & \textbf{R1} & \textbf{R2} & \textbf{RL} \\ \hline
%\multirow{6}{*}{\rotatebox[origin=c]{90}{\small Model Variants}} & F1-level1 & %\textbf{29.38} & 5.13 & \textbf{17.75} \\
% & F1-top & 28.0 & 5.07 & 17.61 \\
% & Recall-level1 & 27.47 & \textbf{5.23} & 17.0 \\
% & Recall-top & 18.37 & 4.04 & 12.4 \\
% & F2-level1 & 26.37 & 4.43 & 16.9 \\
% & F2-top & 25.08 & 4.35 & 16.3 \\ \hline
%\multirow{5}{*}{\rotatebox[origin=c]{90}{\small Baselines}} & Multi-Lead-1 & %25.4 & 3.23 & 14.07 \\
% & Cluster + Best Recall & 21.23 & 3.32 & 13.59 \\
% & Best Word Overlap & 21.43 & 2.83 & 12.96 \\
% & Best F1 & 18.93 & 2.79 & 12.42 \\
% & Cluster + Best F1 & 18.94 & 2.77 & 12.23 \\
%\end{tabular}%
%}
%\caption{ROUGE $F_1$ scores (ROUGE-1, ROUGE-2 and ROUGE-L) on six variants of our model and the baselines on the Camera category. The model variant name indicates the ROUGE-1 metric used for extracting the centroid of each cluster, and the hierarchical level from which the summary is taken.}
%\label{tab_resultsRouge}
%\end{table}

==> figures/tableScoresRougeOther2.tex <==
\begin{table*}[t]
\centering

\begin{tabular}{ll|ll|ll|ll}
 &  & \multicolumn{6}{c}{\textbf{Toys}} \\ \cline{3-8} 
 & \textbf{Model} & \multicolumn{2}{c|}{\textbf{ROUGE-1}} & \multicolumn{2}{c|}{\textbf{ROUGE-2}} & \multicolumn{2}{c}{\textbf{ROUGE-L}} \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\small Variants}} & F1-level1 & \textbf{29.26} & (\textpm 1.87) & 4.64 & (\textpm 0.818) & \textbf{18.24} & (\textpm 1.08) \\
 & F1-top & 27.43 & (\textpm 1.68) & \textbf{4.86} & (\textpm 0.681) & 17.48 & (\textpm 1.1) \\
 & Recall-level1 & 27.57 & (\textpm 1.7) & 4.32 & (\textpm 0.73) & 17.03 & (\textpm 1.09) \\
 & Recall-top & 23.92 & (\textpm 1.74) & 4.31 & (\textpm 0.62) & 15.29 & (\textpm 1.23) \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\small Baselines}} & Multi-Lead-1 & 24.6 & (\textpm 1.0) & 3.17 & (\textpm 0.5) & 14.09 & (\textpm 0.56) \\
 & Best Recall & 23.46 & (\textpm 2.0) & 3.22 & (\textpm 0.67) & 14.0 & (\textpm 1.32) \\
 & Cluster + Best Recall & 21.15 & (\textpm 2.62) & 2.53 & (\textpm 0.49) & 13.47 & (\textpm 1.21) \\
 & Best F1 & 18.57 & (\textpm 3.81) & 2.40 & (\textpm 0.52) & 12.1 & (\textpm 1.82) \\
 & Cluster + Best F1 & 19.27 & (\textpm 3.73) & 2.37 & (\textpm 0.48) & 12.35 & (\textpm 1.7)
\end{tabular}

\caption{ROUGE $F_1$ scores on variants of our model and the baselines, on the Toys category.}
\label{tab_resultsRougeToys}
\end{table*}



\begin{table*}[t]
\centering

\begin{tabular}{ll|ll|ll|ll}
 &  & \multicolumn{6}{c}{\textbf{Electronics}} \\ \cline{3-8} 
 & \textbf{Model} & \multicolumn{2}{c|}{\textbf{ROUGE-1}} & \multicolumn{2}{c|}{\textbf{ROUGE-2}} & \multicolumn{2}{c}{\textbf{ROUGE-L}} \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\small Variants}} & F1-level1 & \textbf{28.81} & (\textpm 1.11) & \textbf{4.77} & (\textpm 0.61) & \textbf{17.47} & (\textpm 0.8) \\
 & F1-top & 26.19 & (\textpm 1.54) & 3.89 & (\textpm 0.57) & 15.82 & (\textpm 0.95) \\
 & Recall-level1 & 27.82 & (\textpm 1.39) & 4.48 & (\textpm 0.6) & 17.43 & (\textpm 0.83) \\
 & Recall-top & 24.15 & (\textpm 1.49) & 4.05 & (\textpm 0.48) & 15.15 & (\textpm 0.88) \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\small Baselines}} & Multi-Lead-1 & 22.83 & (\textpm 1.13) & 2.12 & (\textpm 0.41) & 12.78 & (\textpm 0.54) \\
 & Best Recall & 19.56 & (\textpm 1.48) & 2.13 & (\textpm 0.27) & 11.37 & (\textpm 0.72) \\
 & Cluster + Best Recall & 20.77 & (\textpm 2.31) & 1.82 & (\textpm 0.37) & 12.42 & (\textpm 1.07) \\
 & Best F1 & 19.08 & (\textpm 2.93) & 2.07 & (\textpm 0.47) & 11.94 & (\textpm 1.34) \\
 & Cluster + Best F1 & 20.51 & (\textpm 2.57) & 1.96 & (\textpm 0.43) & 12.53 & (\textpm 1.28)
\end{tabular}

\caption{ROUGE $F_1$ scores on variants of our model and the baselines, on the Electronics category.}
\label{tab_resultsRougeElectronics}
\end{table*}



\begin{table*}[t]
\centering

\begin{tabular}{ll|ll|ll|ll}
 &  & \multicolumn{6}{c}{\textbf{Movies}} \\ \cline{3-8} 
 & \textbf{Model} & \multicolumn{2}{c|}{\textbf{ROUGE-1}} & \multicolumn{2}{c|}{\textbf{ROUGE-2}} & \multicolumn{2}{c}{\textbf{ROUGE-L}} \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\small Variants}} & F1-level1 & 23.99 & (\textpm 1.6) & 4.15 & (\textpm 0.58) & 15.61 & (\textpm 0.98) \\
 & F1-top & 25.26 & (\textpm 1.5) & 4.36 & (\textpm 0.55) & 16.16 & (\textpm 0.8) \\
 & Recall-level1 & \textbf{26.75} & (\textpm 1.35) & \textbf{4.68} & (\textpm 0.49) & \textbf{16.37} & (\textpm 0.86) \\
 & Recall-top & 20.13 & (\textpm 1.46) & 3.96 & (\textpm 0.47) & 12.59 & (\textpm 0.88) \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\small Baselines}} & Multi-Lead-1 & 24.41 & (\textpm 1.1) & 3.56 & (\textpm 0.56) & 14.03 & (\textpm 0.66) \\
 & Best Recall & 22.43 & (\textpm 2.41) & 3.29 & (\textpm 0.61) & 13.49 & (\textpm 1.37) \\
 & Cluster + Best Recall & 15.91 & (\textpm 3.37) & 2.14 & (\textpm 0.59) & 10.49 & (\textpm 1.82) \\
 & Best F1 & 13.67 & (\textpm 3.77) & 2.08 & (\textpm 0.57) & 9.31 & (\textpm 2.17) \\
 & Cluster + Best F1 & 13.43 & (\textpm 3.68) & 1.76 & (\textpm 0.57) & 9.07 & (\textpm 2.1)
\end{tabular}

\caption{ROUGE $F_1$ scores on variants of our model and the baselines, on the Movies category.}
\label{tab_resultsRougeMovies}
\end{table*}




%Toys
%29.26 & (\textpm 1.87) & 4.64 & (\textpm 0.818) & 18.24 & (\textpm 1.08)
%27.43 & (\textpm 1.68) & 4.86 & (\textpm 0.681) & 17.48 & (\textpm 1.1)
%27.57 & (\textpm 1.7) & 4.32 & (\textpm 0.73) & 17.03 & (\textpm 1.09)
%23.92 & (\textpm 1.74) & 4.31 & (\textpm 0.62) & 15.29 & (\textpm 1.23)
%
%24.6 & (\textpm 1.0) & 3.17 & (\textpm 0.5) & 14.09 & (\textpm 0.56)
%23.46 & (\textpm 2.0) & 3.22 & (\textpm 0.67) & 14.0 & (\textpm 1.32)
%21.15 & (\textpm 2.62) & 2.53 & (\textpm 0.49) & 13.47 & (\textpm 1.21)
%18.57 & (\textpm 3.81) & 2.40 & (\textpm 0.52) & 12.1 & (\textpm 1.82)
%19.27 & (\textpm 3.73) & 2.37 & (\textpm 0.48) & 12.35 & (\textpm 1.7)
%
%
%Electronics
%28.81 & (\textpm 1.11) & 4.77 & (\textpm 0.61) & 17.47 & (\textpm 0.8)
%26.19 & (\textpm 1.54) & 3.89 & (\textpm 0.57) & 15.82 & (\textpm 0.95)
%27.82 & (\textpm 1.39) & 4.48 & (\textpm 0.6) & 17.43 & (\textpm 0.83)
%24.15 & (\textpm 1.49) & 4.05 & (\textpm 0.48) & 15.15 & (\textpm 0.88)
%
%22.83 & (\textpm 1.13) & 2.12 & (\textpm 0.41) & 12.78 & (\textpm 0.54)
%19.56 & (\textpm 1.48) & 2.13 & (\textpm 0.27) & 11.37 & (\textpm 0.72)
%20.77 & (\textpm 2.31) & 1.82 & (\textpm 0.37) & 12.42 & (\textpm 1.07)
%19.08 & (\textpm 2.93) & 2.07 & (\textpm 0.47) & 11.94 & (\textpm 1.34)
%20.51 & (\textpm 2.57) & 1.96 & (\textpm 0.43) & 12.53 & (\textpm 1.28)
%
%
%
%Movies
%23.99 & (\textpm 1.6) & 4.15 & (\textpm 0.58) & 15.61 & (\textpm 0.98)
%25.26 & (\textpm 1.5) & 4.36 & (\textpm 0.55) & 16.16 & (\textpm 0.8)
%26.75 & (\textpm 1.35) & 4.68 & (\textpm 0.49) & 16.37 & (\textpm 0.86)
%20.13 & (\textpm 1.46) & 3.96 & (\textpm 0.47) & 12.59 & (\textpm 0.88)
%
%24.41 & (\textpm 1.1) & 3.56 & (\textpm 0.56) & 14.03 & (\textpm 0.66)
%22.43 & (\textpm 2.41) & 3.29 & (\textpm 0.61) & 13.49 & (\textpm 1.37)
%15.91 & (\textpm 3.37) & 2.14 & (\textpm 0.59) & 10.49 & (\textpm 1.82)
%13.67 & (\textpm 3.77) & 2.08 & (\textpm 0.57) & 9.31 & (\textpm 2.17)
%13.43 & (\textpm 3.68) & 1.76 & (\textpm 0.57) & 9.07 & (\textpm 2.1)
%
%
%Music
%Baselines
%25.22 & (\textpm 1.4) & 3.12 & (\textpm 0.51) & 13.92 & (\textpm 0.78)
%20.56 & (\textpm 2.03) & 2.12 & (\textpm 0.35) & 11.66 & (\textpm 0.99)
%18.69 & (\textpm 2.66) & 2.04 & (\textpm 0.57) & 11.62 & (\textpm 1.43)
%17.08 & (\textpm 3.5) & 2.15 & (\textpm 0.71) & 10.96 & (\textpm 1.96)
%14.97 & (\textpm 3.74) & 2.08 & (\textpm 0.77) & 10.12 & (\textpm 2.19)



==> figures/tableScoresRougeOther3.tex <==
\begin{table*}[]
\centering

\begin{tabular}{ll|ll|ll|ll}
 &  & \multicolumn{6}{c}{\textbf{Toys}} \\ \cline{3-8} 
 & \textbf{Model} & \multicolumn{2}{c|}{\textbf{ROUGE-1}} & \multicolumn{2}{c|}{\textbf{ROUGE-2}} & \multicolumn{2}{c}{\textbf{ROUGE-L}} \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\small Variants}} & level1-F1 & \textbf{29.26} & (\textpm 1.87) & 4.64 & (\textpm 0.818) & \textbf{18.24} & (\textpm 1.08) \\
 & level1-Recall & 27.57 & (\textpm 1.7) & 4.32 & (\textpm 0.73) & 17.03 & (\textpm 1.09) \\
 & top-F1 & 27.43 & (\textpm 1.68) & \textbf{4.86} & (\textpm 0.681) & 17.48 & (\textpm 1.1) \\
 & top-Recall & 23.92 & (\textpm 1.74) & 4.31 & (\textpm 0.62) & 15.29 & (\textpm 1.23) \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\small Baselines}} & Medoid-F1 & 28.41 & (\textpm 1.44) & 3.9 & (\textpm 0.6) & 16.59 & (\textpm 1.01) \\
 & Cluster + Medoid-F1 & 25.22 & (\textpm 2.84) & 3.76 & (\textpm 0.7) & 15.32 & (\textpm 1.4) \\
 & Multi-Lead-1 & 24.72 & (\textpm 1.12) & 3.30 & (\textpm 0.58) & 14.36 & (\textpm 0.65) \\
 & Cluster + Medoid-Recall & 19.57 & (\textpm 1.62) & 2.73 & (\textpm 0.42) & 11.37 & (\textpm 0.84) \\
 & Medoid-Recall & 16.99 & (\textpm 1.37) & 2.52 & (\textpm 0.33) & 9.92 & (\textpm 0.76)
\end{tabular}

\caption{ROUGE $F_1$ scores on variants of our model and the baselines, on the Toys category.}
\label{tab_resultsRougeToys}
\end{table*}



\begin{table*}[]
\centering

\begin{tabular}{ll|ll|ll|ll}
 &  & \multicolumn{6}{c}{\textbf{Camera}} \\ \cline{3-8} 
 & \textbf{Model} & \multicolumn{2}{c|}{\textbf{ROUGE-1}} & \multicolumn{2}{c|}{\textbf{ROUGE-2}} & \multicolumn{2}{c}{\textbf{ROUGE-L}} \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\small Variants}} & level1-F1 & \textbf{29.25} & (\textpm 1.45) & 5.26 & (\textpm 0.69) & \textbf{17.74} & (\textpm 0.76) \\
 & level1-Recall & 27.94 & (\textpm 1.53) & \textbf{5.36} & (\textpm 0.61) & 17.18 & (\textpm 0.74) \\
 & top-F1 & 27.5 & (\textpm 1.88) & 5.06 & (\textpm 0.76) & 17.37 & (\textpm 0.94) \\
 & top-Recall & 18.77 & (\textpm 1.95) & 4.13 & (\textpm 0.5) & 12.62 & (\textpm 0.91) \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\small Baselines}} & Medoid-F1 & 28.27 & (\textpm 1.53) & 4.05 & (\textpm 0.65) & 16.6 & (\textpm 0.86) \\
 & Cluster + Medoid-F1 & 27.33 & (\textpm 1.68) & 3.44 & (\textpm 0.51) & 15.69 & (\textpm 0.74) \\
 & Multi-Lead-1 & 25.85 & (\textpm 1.57) & 3.65 & (\textpm 0.70) & 14.81 & (\textpm 0.78) \\
 & Cluster + Medoid-Recall & 20.95 & (\textpm 1.87) & 2.83 & (\textpm 0.45) & 12.29 & (\textpm 1.09) \\
 & Medoid-Recall & 16.17 & (\textpm 1.64) & 2.69 & (\textpm 0.52) & 9.52 & (\textpm 0.83)
\end{tabular}

\caption{ROUGE $F_1$ scores on variants of our model and the baselines, on the Camera category.}
\label{tab_resultsRougeCamera}
\end{table*}



\begin{table*}[]
\centering

\begin{tabular}{ll|ll|ll|ll}
 &  & \multicolumn{6}{c}{\textbf{DVDs}} \\ \cline{3-8} 
 & \textbf{Model} & \multicolumn{2}{c|}{\textbf{ROUGE-1}} & \multicolumn{2}{c|}{\textbf{ROUGE-2}} & \multicolumn{2}{c}{\textbf{ROUGE-L}} \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\small Variants}} & level1-F1 & 23.99 & (\textpm 1.6) & 4.15 & (\textpm 0.58) & 15.61 & (\textpm 0.98) \\
 & level1-Recall & \textbf{26.75} & (\textpm 1.35) & \textbf{4.68} & (\textpm 0.49) & \textbf{16.37} & (\textpm 0.86) \\
 & top-F1 & 25.26 & (\textpm 1.5) & 4.36 & (\textpm 0.55) & 16.16 & (\textpm 0.8) \\
 & top-Recall & 20.13 & (\textpm 1.46) & 3.96 & (\textpm 0.47) & 12.59 & (\textpm 0.88) \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\small Baselines}} & Medoid-F1 & 26.16 & (\textpm 1.39) & 4.14 & (\textpm 0.5) & 15.27 & (\textpm 0.71) \\
 & Cluster + Medoid-F1 & 24.94 & (\textpm 1.37) & 3.56 & (\textpm 0.44) & 14.75 & (\textpm 0.59) \\
 & Multi-Lead-1 & 24.93 & (\textpm 1.36) & 3.41 & (\textpm 0.50) & 14.49 & (\textpm 0.77) \\
 & Cluster + Medoid-Recall & 21.43 & (\textpm 1.08) & 3.25 & (\textpm 0.31) & 11.85 & (\textpm 0.69) \\
 & Medoid-Recall & 18.72 & (\textpm 1.01) & 3.11 & (\textpm 0.28) & 10.41 & (\textpm 0.62)
\end{tabular}

\caption{ROUGE $F_1$ scores on variants of our model and the baselines, on the DVDs category.}
\label{tab_resultsRougeMovies}
\end{table*}






%Toys
%29.26 & (\textpm 1.87) & 4.64 & (\textpm 0.818) & 18.24 & (\textpm 1.08)
%27.43 & (\textpm 1.68) & 4.86 & (\textpm 0.681) & 17.48 & (\textpm 1.1)
%27.57 & (\textpm 1.7) & 4.32 & (\textpm 0.73) & 17.03 & (\textpm 1.09)
%23.92 & (\textpm 1.74) & 4.31 & (\textpm 0.62) & 15.29 & (\textpm 1.23)
%
%24.6 & (\textpm 1.0) & 3.17 & (\textpm 0.5) & 14.09 & (\textpm 0.56)
%23.46 & (\textpm 2.0) & 3.22 & (\textpm 0.67) & 14.0 & (\textpm 1.32)
%21.15 & (\textpm 2.62) & 2.53 & (\textpm 0.49) & 13.47 & (\textpm 1.21)
%18.57 & (\textpm 3.81) & 2.40 & (\textpm 0.52) & 12.1 & (\textpm 1.82)
%19.27 & (\textpm 3.73) & 2.37 & (\textpm 0.48) & 12.35 & (\textpm 1.7)
%
%
%Electronics
%28.81 & (\textpm 1.11) & 4.77 & (\textpm 0.61) & 17.47 & (\textpm 0.8)
%26.19 & (\textpm 1.54) & 3.89 & (\textpm 0.57) & 15.82 & (\textpm 0.95)
%27.82 & (\textpm 1.39) & 4.48 & (\textpm 0.6) & 17.43 & (\textpm 0.83)
%24.15 & (\textpm 1.49) & 4.05 & (\textpm 0.48) & 15.15 & (\textpm 0.88)
%
%22.83 & (\textpm 1.13) & 2.12 & (\textpm 0.41) & 12.78 & (\textpm 0.54)
%19.56 & (\textpm 1.48) & 2.13 & (\textpm 0.27) & 11.37 & (\textpm 0.72)
%20.77 & (\textpm 2.31) & 1.82 & (\textpm 0.37) & 12.42 & (\textpm 1.07)
%19.08 & (\textpm 2.93) & 2.07 & (\textpm 0.47) & 11.94 & (\textpm 1.34)
%20.51 & (\textpm 2.57) & 1.96 & (\textpm 0.43) & 12.53 & (\textpm 1.28)
%
%
%
%Movies
%23.99 & (\textpm 1.6) & 4.15 & (\textpm 0.58) & 15.61 & (\textpm 0.98)
%25.26 & (\textpm 1.5) & 4.36 & (\textpm 0.55) & 16.16 & (\textpm 0.8)
%26.75 & (\textpm 1.35) & 4.68 & (\textpm 0.49) & 16.37 & (\textpm 0.86)
%20.13 & (\textpm 1.46) & 3.96 & (\textpm 0.47) & 12.59 & (\textpm 0.88)
%
%24.41 & (\textpm 1.1) & 3.56 & (\textpm 0.56) & 14.03 & (\textpm 0.66)
%22.43 & (\textpm 2.41) & 3.29 & (\textpm 0.61) & 13.49 & (\textpm 1.37)
%15.91 & (\textpm 3.37) & 2.14 & (\textpm 0.59) & 10.49 & (\textpm 1.82)
%13.67 & (\textpm 3.77) & 2.08 & (\textpm 0.57) & 9.31 & (\textpm 2.17)
%13.43 & (\textpm 3.68) & 1.76 & (\textpm 0.57) & 9.07 & (\textpm 2.1)
%
%
%Music
%Baselines
%25.22 & (\textpm 1.4) & 3.12 & (\textpm 0.51) & 13.92 & (\textpm 0.78)
%20.56 & (\textpm 2.03) & 2.12 & (\textpm 0.35) & 11.66 & (\textpm 0.99)
%18.69 & (\textpm 2.66) & 2.04 & (\textpm 0.57) & 11.62 & (\textpm 1.43)
%17.08 & (\textpm 3.5) & 2.15 & (\textpm 0.71) & 10.96 & (\textpm 1.96)
%14.97 & (\textpm 3.74) & 2.08 & (\textpm 0.77) & 10.12 & (\textpm 2.19)



==> figures/tableSummaryLengths.tex <==
\begin{table*}[ht!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|cc|cc|cc|cc|cc|cc}
                           &                       & \multicolumn{2}{c|}{\textbf{Electronics}} & \multicolumn{2}{c|}{\textbf{Books}} & \multicolumn{2}{c|}{\textbf{Toys}} & \multicolumn{2}{c|}{\textbf{Camera}} & \multicolumn{2}{c|}{\textbf{DVDs}} & \multicolumn{2}{c}{\textbf{Music}} \\
                           &                       & \textbf{mean}      & \textbf{med}      & \textbf{mean}   & \textbf{med}   & \textbf{mean}   & \textbf{med}  & \textbf{mean}    & \textbf{med}   & \textbf{mean}    & \textbf{med}   & \textbf{mean}   & \textbf{med}   \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\small Variants}}  & level1-F1             & 70.27              & 69                   & 48.25           & 47                & 58.15           & 55.5             & 47.15            & 48.5              & 38.14            & 40                & -               & -                 \\
                           & level1-Recall         & 79.64              & 80                   & 78.85           & 78                & 65.68           & 68               & 94.0             & 87.5              & 106.65           & 102               & -               & -                 \\
                           & top-F1                & 80.09              & 80                   & 41.5            & 39                & 71.55           & 60.5             & 42.3             & 40                & 62.81            & 57                & -               & -                 \\
                           & top-Recall            & 126.91             & 115                  & 164.4           & 162.5             & 116.84          & 102              & 242.25           & 249.5             & 237.45           & 237.5             & -               & -                 \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\small Baselines}} & Best F1               & 68.55              & 72.5                 & 55.25           & 42.5              & 61.7            & 50.5             & 71.8             & 65.5              & 59.14            & 55                & 77.9            & 76.5              \\
                           & Cluster + Best F1     & 77.91              & 71.5                 & 61.65           & 63.5              & 53.8            & 44.5             & 82.9             & 70.5              & 61.52            & 63                & 76.8            & 70                \\
                           & Multi-Lead-1          & 88.14              & 92.5                 & 85.2            & 92.5              & 90.8            & 92               & 89.0             & 92.5              & 87.05            & 89                & 78.85           & 87.5              \\
                           & Cluster + Best Recall & 277.27             & 278                  & 206.4           & 193               & 226.1           & 234.5            & 220.3            & 227.5             & 301.0            & 298               & 318.25          & 318.5             \\
                           & Best Recall           & 378.59             & 396.5                & 313.2           & 311               & 333.85          & 350              & 364.75           & 384               & 386.19           & 405               & 374.25          & 421               \\ \hline
                           & Test Reviews          & 67.07              & 41                   & 56.35           & 32                & 56.29           & 34               & 77.73            & 50                & 67.75            & 36                & 89.04           & 54
\end{tabular}%
}
\caption{Average and median number of tokens in the summaries analyzed and in the reviews of the test set.}
\label{tab_summaryLens}


\vspace{8em}


\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|cc|cc|cc|cc|cc|cc}
                           &                       & \multicolumn{2}{c|}{\textbf{Electronics}} & \multicolumn{2}{c|}{\textbf{Books}} & \multicolumn{2}{c|}{\textbf{Toys}} & \multicolumn{2}{c|}{\textbf{Camera}} & \multicolumn{2}{c|}{\textbf{DVDs}} & \multicolumn{2}{c}{\textbf{Music}} \\
                           &                       & \textbf{vsMean}      & \textbf{vsMed}     & \textbf{vsMean}   & \textbf{vsMed}  & \textbf{vsMean}  & \textbf{vsMed}  & \textbf{vsMean}   & \textbf{vsMed}   & \textbf{vsMean}   & \textbf{vsMed}   & \textbf{vsMean}   & \textbf{vsMed}  \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\small Variants}}  & level1-F1             & 1.09                 & 1.71               & 0.97              & 1.6             & 1.12             & 1.87            & 0.75              & 1.07             & 0.58              & 1.06             & -                 & -               \\
                           & level1-Recall         & 1.23                 & 1.93               & 1.58              & 2.59            & 1.20             & 2.01            & 1.48              & 2.13             & 1.56              & 2.85             & -                 & -               \\
                           & top-F1                & 1.25                 & 1.97               & 0.82              & 1.39            & 1.27             & 2.07            & 0.65              & 0.94             & 0.96              & 1.77             & -                 & -               \\
                           & top-Recall            & 1.92                 & 3.04               & 3.24              & 5.33            & 2.33             & 3.87            & 3.56              & 5.1              & 3.63              & 6.69             & -                 & -               \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\small Baselines}} & Best F1               & 1.02                 & 1.61               & 0.99              & 1.64            & 1.03             & 1.67            & 0.95              & 1.36             & 0.84              & 1.52             & 0.91              & 1.56            \\
                           & Cluster + Best F1     & 1.16                 & 1.87               & 1.16              & 1.88            & 0.87             & 1.39            & 1.10              & 1.59             & 0.87              & 1.55             & 0.87              & 1.45            \\
                           & Multi-Lead-1          & 1.40                 & 2.16               & 1.77              & 2.83            & 1.77             & 2.95            & 1.44              & 2.07             & 1.30              & 2.37             & 1.00              & 1.78            \\
                           & Cluster + Best Recall & 4.14                 & 6.61               & 3.73              & 6.38            & 3.85             & 6.41            & 2.93              & 4.21             & 4.43              & 8.15             & 3.89              & 6.87            \\
                           & Best Recall           & 5.83                 & 9.24               & 6.10              & 10.18           & 6.18             & 10.24           & 5.39              & 7.70             & 5.65              & 10.39            & 4.66              & 8.18
\end{tabular}%
}
\caption{The average compression ratios of summaries analyzed against their respective reviews. Each summary's token-length is divided by either the mean or median review token-length of its corresponding review set.}
\label{tab_compressionRatios}



\end{table*}




                        
                        
%                        Electronics     Books           Toys            Camera          Movies          Music
%baseline                mean    median  mean    median  mean    median  mean    median  mean    median  mean    median
%Best F1	                68.55	72.5    55.25	42.5	61.7	50.5    71.8	65.5    59.14	55.0    77.9	76.5
%Cluster + Best F1	    77.91	71.5    61.65	63.5	53.8	44.5    82.9	70.5    61.52	63.0    76.8	70.0
%Multi-Lead-1	        88.14	92.5    85.2	92.5	90.8	92.0    89.0	92.5    87.05	89.0    78.85	87.5
%Cluster + Best Recall   277.27	278   206.4	193	226.1	234.5   220.3	227.5   301.0	298.0   318.25	318.5
%Best Recall	            378.59	396.5   313.2	311.0	333.85	350.0   364.75	384.0   386.19	405.0   374.25	421.0
%level1-F1               70.27	69.0    48.25	47.0    58.15	55.5    47.15	48.5    38.14	40.0
%level1-Recall           79.64	80.0    78.85	78.0    65.68	68.0    94.0	87.5    106.65	102.0
%top-F1                  80.09	80.0    41.5	39.0    71.55	60.5    42.3	40.0    62.81	57.0
%top-Recall              126.91	115.0   164.4	162.5   116.84	102.0   242.25	249.5   237.45	237.5
%Review Lengths          67.07	41.0    56.35	32.0	56.29	34.0    77.73	50.0    67.75	36.0    89.04	54.0
%
%
%                        Electronics     Books           Toys            Camera          Movies          Music
%baseline                vsMean  vsMed   vsMean  vsMed   vsMean  vsMed   vsMean  vsMed   vsMean  vsMed   vsMean  vsMed
%Best F1	                1.02    1.61    0.99    1.64    1.03    1.67    0.95    1.36    0.84    1.52    0.91    1.56
%Cluster + Best F1	    1.16    1.87    1.16    1.88    0.87    1.39    1.10    1.59    0.87    1.55    0.87    1.45
%Multi-Lead-1	        1.40    2.16    1.77    2.83    1.77    2.95    1.44    2.07    1.30    2.37    1.00    1.78
%Cluster + Best Recall   4.14    6.61    3.73    6.38    3.85    6.41    2.93    4.21    4.43    8.15    3.89    6.87
%Best Recall	            5.83    9.24    6.10    10.18   6.18    10.24   5.39    7.70    5.65    10.39   4.66    8.18
%level1-F1               1.09	1.71    0.97	1.6     1.12	1.87    0.75	1.07    0.58	1.06
%level1-Recall           1.23	1.93    1.58	2.59    1.20	2.01    1.48	2.13    1.56	2.85
%top-F1                  1.25	1.97    0.82	1.39    1.27	2.07    0.65	0.94    0.96	1.77
%top-Recall              1.92	3.04    3.24	5.33    2.33	3.87    3.56	5.1     3.63	6.69
                        

            




%Electronics
%baseline	            min	max	mean	median	ratioAsMean	ratioAsMedian
%Best F1	                25	144	68.55	72.5	1.02	    1.61
%Cluster + Best F1	    22	162	77.91	71.5	1.16	    1.87
%Multi-Lead-1	        31	100	88.14	92.5	1.40	    2.16
%Cluster + Best Recall	76	443	277.27	278.0	4.14	    6.61
%Best Recall	            202	453	378.59	396.5	5.83	    9.24
%Review Lengths          1	474	67.07	41.0	
%
%Books
%baseline	            min	max	mean	median	ratioAsMean	ratioAsMedian
%Best F1	                19	121	55.25	42.5	0.99	    1.64
%Cluster + Best F1	    25	129	61.65	63.5	1.16	    1.88
%Multi-Lead-1	        51	100	85.2	92.5	1.77	    2.83
%Cluster + Best Recall	62	404	206.4	193.0	3.73	    6.38
%Best Recall	            124	452	313.2	311.0	6.10	    10.18
%Review Lengths          1	456	56.35	32.0	
%
%Toys
%baseline	            min	max	mean	median	ratioAsMean	ratioAsMedian
%Best F1	                24	152	61.7	50.5	1.03	    1.67
%Cluster + Best F1	    5	119	53.8	44.5	0.87	    1.39
%Multi-Lead-1	        67	100	90.8	92.0	1.77	    2.95
%Cluster + Best Recall	39	419	226.1	234.5	3.85	    6.41
%Best Recall	            93	483	333.85	350.0	6.18	    10.24
%Review Lengths          1	489	56.29	34.0
%
%Camera
%baseline	            min	max	mean	median	ratioAsMean	ratioAsMedian
%Best F1	                19	139	71.8	65.5	0.95	    1.36
%Cluster + Best F1	    28	216	82.9	70.5	1.10	    1.59
%Multi-Lead-1	        58	100	89.0	92.5	1.44	    2.07
%Cluster + Best Recall	27	451	220.3	227.5	2.93	    4.21
%Best Recall	            141	457	364.75	384.0	5.39	    7.70
%Review Lengths          1	462	77.73	50.0	
%
%Movies
%baseline	            min	max	mean	median	ratioAsMean	ratioAsMedian
%Best F1	                18	99	59.14	55.0	0.84	    1.52
%Cluster + Best F1	    18	164	61.52	63.0	0.87	    1.55
%Multi-Lead-1	        53	100	87.05	89.0	1.30	    2.37
%Cluster + Best Recall	174	462	301.0	298.0	4.43	    8.15
%Best Recall	            222	469	386.19	405.0	5.65	    10.39
%Review Lengths          1	469	67.75	36.0	
%
%Music
%baseline	            min	max	mean	median	ratioAsMean	ratioAsMedian
%Best F1	                22	186	77.9	76.5	0.91	    1.56
%Cluster + Best F1	    22	202	76.8	70.0	0.87	    1.45
%Multi-Lead-1	        0	100	78.85	87.5	1.00	    1.78
%Cluster + Best Recall	99	504	318.25	318.5	3.89	    6.87
%Best Recall	            159	504	374.25	421.0	4.66	    8.18
%Review Lengths          1	581	89.04	54.0

%variant	                    min	max	mean	median	ratioAsMean	ratioAsMedian
%Electronics_level1-F1	    41	105	70.27	69.0	1.09	1.71
%Electronics_level1-Recall	42	113	79.64	80.0	1.23	1.93
%Electronics_top-F1	        41	120	80.09	80.0	1.25	1.97
%Electronics_top-Recall	    66	197	126.91	115.0	1.92	3.04
%Books_level1-F1	            30	75	48.25	47.0	0.97	1.6
%Books_level1-Recall	        52	123	78.85	78.0	1.58	2.59
%Books_top-F1	            17	71	41.5	39.0	0.82	1.39
%Books_top-Recall	        64	253	164.4	162.5	3.24	5.33
%Toys_level1-F1	            41	84	58.15	55.5	1.12	1.87
%Toys_level1-Recall	        26	102	65.68	68.0	1.20	2.01
%Toys_top-F1	                31	153	71.55	60.5	1.27	2.07
%Toys_top-Recall	            35	234	116.84	102.0	2.33	3.87
%Camera_level1-F1	        30	57	47.15	48.5	0.75	1.07
%Camera_level1-Recall	    61	141	94.0	87.5	1.48	2.13
%Camera_top-F1	            20	70	42.3	40.0	0.65	0.94
%Camera_top-Recall	        71	403	242.25	249.5	3.56	5.1
%Movies_level1-F1	        14	54	38.14	40.0	0.58	1.06
%Movies_level1-Recall	    60	180	106.65	102.0	1.56	2.85
%Movies_top-F1	            27	112	62.81	57.0	0.96	1.77
%Movies_top-Recall	        103	535	237.45	237.5	3.63	6.69

==> figures/tablesScoresManual2.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|lllll}
\textbf{Model} & \textbf{Q1} & \textbf{Q2} & \textbf{Q3} & \textbf{Q4} & \textbf{Q5} \\ \hline
Ours & \textbf{3.85} & 3.55 & \textbf{3.90} & \textbf{4.15} & 3.90 \\
Best Recall & 3.40 & \textbf{3.80} & \textbf{3.90} & 3.95 & \textbf{4.00} \\
Multi-Lead-1 &  3.05 & 2.95 & 3.50 & 3.10 & 3.10 \\
\end{tabular}%
}

\caption{Manual coherence scores on our system (F1-level1 variant) and two relatively strong baselines, on the Camera category. Generally, the criteria are: (Q1) grammaticality, (Q2) non-redundancy, (Q3) referential clarity, (Q4) focus, and (Q5) structure and coherence. Notice that the \textit{Best Recall} ``summaries'' are human-written reviews, hence linguistic quality should be high.}
\label{tab_resultsResponsiveness}
\end{table}

==> figures/tablesScoresManualPrev.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc}
\textbf{Criterion} & \textbf{Ours} & \textbf{Best Rec.} & \textbf{M-L-1} \\ \hline
Grammaticality & \textbf{3.85} & 3.40 & 3.05 \\
Non-redundancy & 3.55 & \textbf{3.80} & 2.95 \\
Referential clarity & \textbf{3.90} & \textbf{3.90} & 3.50 \\
Focus & \textbf{4.15} & 3.95 & 3.10 \\
Structure \& coherence & 3.90 & \textbf{4.00} & 3.10 \\
\end{tabular}%
}

\caption{Manual coherence scores on our system (level1-F1 variant) and the \textit{Best Recall} and \textit{Multi-Lead-1} baselines, on the Camera category.
%Notice that the \textit{Best Recall} ``summaries'' are human-written reviews, hence linguistic quality should be high.
}
\label{tab_resultsResponsiveness}
\end{table}
